Layer-wise Analysis of a Self-supervised Speech Representation Model

Recently proposed self-supervised learning approaches have been successful for pre-training speech representation models. The utility of these learned representations has been observed empirically, but not much has been studied about the type or extent of information encoded in the pre-trained representations themselves. Developing such insights can help understand the capabilities and limits of these models and enable the research community to more efficiently develop their usage for downstream applications. In this work, we begin to fill this gap by examining one recent and successful pre-trained model (wav2vec 2.0), via its intermediate representation vectors, using a suite of analysis tools. We use the metrics of canonical correlation, mutual information, and performance on simple downstream tasks with non-parametric probes, in order to (i) query for acoustic and linguistic information content, (ii) characterize the evolution of information across model layers, and (iii) understand how fine-tuning the model for automatic speech recognition (ASR) affects these observations. Our findings motivate modifying the fine-tuning protocol for ASR, which produces improved word error rates in a low-resource setting.

==> table.tex <==
\begin{table}[]
\centering
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cr|cc|cc}
%   \centered{\multirow{2}{*}{\bf train set}}  & \centered{\multirow{2}{*}{$n$}} & \multicolumn{2}{c|}{
\multirow{2}{*}{\bf train set}  & \multirow{2}{*}{$n$} & \multicolumn{2}{c|}{
                     %best 
                     %asr-finetune-n} 
                     \bf re-init last 12-$n$ layers}& \multicolumn{2}{c}{
                     %asr-finetune-12
                     \bf standard fine-tuning} \\ \cline{3-6} 
\multicolumn{1}{l}{} &                    & test-clean         & test-other         & test-clean        & test-other       \\ \hline
10m                  & 9                  & 44.1               & 51.8               & 49.0              & 56.7             \\ %\hline
1h                   & 11                 & 19.8               & 29.3               & 20.3              & 29.9             \\ %\hline
10h                  & 11                 & 10.9               & 19.4               & 11.3              & 20.6            
\end{tabular}%
}
\caption{\it Word error rates (\%) for modified fine-tuning protocol, using the best value of $n$ based on dev-clean performance, compared to the standard fine-tuning approach. \kl{it might be nice to reformat the table in the same way we did for the MLSLP poster.  Also, how about "re-init last 12-n layers" $\longrightarrow$ "re-init last n layers"?}\jc{I think it will be a little confusing to for example says n=3} \kl{I think it's clear but I don't have strong feelings about it either way}}
\label{tab:wer_backup}
\vspace{-.1in}
%{\it asr-finetune-12}.} \kl{The table looks much nicer.  I formatted a bit and added a title for the first column.  For reference here is Herman Kamper's writeup style:  https://www.kamperh.com/notes/writing}}
\end{table}
